Advances in the Determination of Quark Masses

Significant progress has been made in the determination of the light quark masses, using both lattice QCD and sum rule methods, in the last year. We discuss the different methods and review the status of current results. Finally, we review the calculations of bottom and charm quark masses.

==> Makefile <==
# %auto-ignore
MAINFILE=  paper.tex

TEXFILES=  espcrc2.sty rgmac.latex t-ape.tex
AXISFILES= f-Wmbar.ax f-mbarstag.ax f-SWimp.ax f-SWTmbar.ax f-NPSWmbar.ax \
	   f-Wms.ax f-SWTms.ax
FIGFILES=  
PSFILES=   
#########################################################################
# special rules if any

#########################################################################
#									#
#                 NO USER SERVICEABLE PARTS BELOW !!!                   #
# 									#
#########################################################################


# List of all the sources
SOURCES= Makefile ${MAINFILE} ${TEXFILES} ${AXISFILES} ${FIGFILES} ${PSFILES}

# List of all postscript figures to be included.
PSINCLUSIONS= ${AXISFILES:.ax=.ps} ${FIGFILES:.fig=.ps} ${PSFILES}

# what is to be made by default
all: ${MAINFILE:.tex=.ps}

# re-dvips if any of these change
${MAINFILE:.tex=.ps}: ${MAINFILE:.tex=.dvi} ${PSINCLUSIONS}

# re-latex if any of these change
${MAINFILE:.tex=.dvi}: ${MAIN} ${TEXFILES} ${PSINCLUSIONS}

# Never try to `make' any of the sources
${SOURCES}:;

# The rest of them do not have any `extra' dependencies, i.e. a.x depends 
# obviously depends on a.y if a.x is to be created from a.y.

.PHONY: clean realclean
# clean removes ~ aux log and tmp files
clean:
	rm -f *~ *.aux *.log *.tmp
# real clean removes everything but sources and final products
realclean: clean
	rm -f ${AXISFILES:.ax=.ps} ${FIGFILES:.fig=.ps}

########################################################################
# General rules of how to build something from something else.
.SUFFIXES: .ps .dvi .tex .ax .xy .fig

# If .fig exists that is how to create ps.
%.ps: %.fig
	fig2dev -L ps $< > $@

# If .ax or .xy exist, that is the source of the .ps file
%.ps: %.ax
	xyplot $< | epsplot > $@.tmp
	sed -e "/%%BoundingBox: /d" -e '1a\
	'"`psbbox $@.tmp`" $@.tmp > $@ 
	rm -f $@.tmp
%.ps: %.xy
	xyplot $< | epsplot > $@.tmp
	sed -e "/%%BoundingBox: /d" -e '1a\
	'"`psbbox $@.tmp`" $@.tmp > $@ 
	rm -f $@.tmp

# else look for a dvi file.
%.ps: %.dvi
	dvips -z -o $@ $<


# dvi is always created from tex.
%.dvi: %.tex
	latex $<
	if grep -i -q rerun ${<:.tex=.log} ; then latex $<; fi

##################################################################

submission: ${SOURCES} ${PSINCLUSIONS}
	(echo "."; \
	 echo "${SOURCES} ${PSINCLUSIONS}" ; \
	 echo "submission") | uufiles -gz -9

